GeoTrackNet-A Maritime Anomaly Detector using Probabilistic Neural Network Representation of AIS Tracks and A Contrario Detection

Representing maritime traffic patterns and detecting anomalies from them are key to vessel monitoring and maritime situational awareness. We propose a novel approach -- referred to as GeoTrackNet -- for maritime anomaly detection from AIS data streams. Our model exploits state-of-the-art neural network schemes to learn a probabilistic representation of AIS tracks and a contrario detection to detect abnormal events. The neural network provides a new means to capture complex and heterogeneous patterns in vessels' behaviours, while the \textit{a contrario} detector takes into account the fact that the learnt distribution may be location-dependent. Experiments on a real AIS dataset comprising more than 4.2 million AIS messages demonstrate the relevance of the proposed method compared with state-of-the-art schemes.

==> bio2.tex <==
\begin{IEEEbiography}
    [{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/biography/Nguyen.jpg}}]{Duong Nguyen}
received the Diplôme d'Ing\'enieur in machine learning from T\'el\'ecom Bretagne, the M.Sc. degree (summa cum laude) in signal and image processing from the University of Rennes 1, and the Ph.D. degree in machine learning from IMT Atlantique. His research interests focus on the study of machine learning (deep learning) for time series modelling and analysis, with applications to dynamical system identification and maritime traffic surveillance.
\end{IEEEbiography}

\begin{IEEEbiography}
    [{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/biography/Nguyen.jpg}}]{Duong Nguyen}
received the Diplôme d'Ing\'enieur in machine learning from T\'el\'ecom Bretagne, the M.Sc. degree (summa cum laude) in signal and image processing from the University of Rennes 1, and the Ph.D. degree in machine learning from IMT Atlantique. His research interests focus on the study of machine learning (deep learning) for time series modelling and analysis, with applications to dynamical system identification and maritime traffic surveillance.
\end{IEEEbiography}

==> biography.tex <==
\begin{IEEEbiography}
    [{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/biography/Nguyen.jpg}}]{Duong Nguyen}
received the Diplôme d'Ing\'enieur in machine learning from T\'el\'ecom Bretagne, the M.Sc. degree (summa cum laude) in signal and image processing from the University of Rennes 1, and the Ph.D. degree in machine learning from IMT Atlantique. 

His research interests focus on the study of machine learning (deep learning) for time series modelling and analysis, with applications to dynamical system identification and maritime traffic surveillance.
\end{IEEEbiography}

\begin{IEEEbiography}
    [{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/biography/Vadaine.jpg}}]{Rodolphe Vadaine}
received the M.Sc. degree in electronics and signal processing from the \'Ecole Nationale Sup\'erieure d'\'Electronique, d'\'Electrotechnique,
d'Informatique, d'Hydraulique et des T\'el\'ecommunications (ENSEEIHT), Toulouse, France, in 2012.

He worked with GEVES (Groupement d'\'Etude des Vari\'et\'es et des Semences) between 2013 and 2015 on the development of news imaging methods for the phenotyping of seeds and plants based on multi-modal imagery. He then joined CLS in 2016, where he has been working on innovative image processing methods based on SAR and optical satellite imagery. He is currently involved in the development of new machine learning algorithms for various applications including oil pollution detection, ship traffic monitoring and sea ice mapping.
\end{IEEEbiography}

\begin{IEEEbiography}
    [{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/biography/Hajduch.jpg}}]{Guillaume Hajduch}
holds degrees in telecommunication engineering and a PhD in signal processing for imaging Radars. He worked in the definition, prototyping and development of airborne radar imaging modes for maritime applications and of maritime products derived from spaceborne Synthetic Aperture Radar. Since 2008 at CLS, he oversees R\&D activities related to monitoring of maritime activities using inter alia Earth Observation, AIS, and UAV observation. He is as well leading the Sentinel-1 Mission Performance Centre (S-1 MPC) consortium, responsible for the European Space Agency of the quality and performances of the Sentinel-1 SAR products. 
\end{IEEEbiography}

\begin{IEEEbiography}
    [{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/biography/Garello.jpg}}]{Ren\'e Garello}
professor at IMT Atlantique, Fellow IEEE, head of the program ICTO (ICT and OCEANS) within the CNRS research unit LabSTICC. 

Ren\'e Garello was born in 1953. He received the Ph.D. degree in Signal Processing at the Institut National Polytechnique de Grenoble (INPG) in 1981. From 1982 to 1984 he worked as a
Research Associate at Aeronomy Lab, National Oceanic and Atmospheric Administration (NOAA) at Boulder, Colorado (USA). He joined the Institut Mines-T\'el\'ecom Atlantique (IMT Atlantique, formerly T\'el\'ecom Bretagne), Brest, France in 1985. In 1988, he became Professor in this engineering school
in the field of signal processing and image processing and in 1995, Prof. Garello obtained his Habilitation (HDR; Habilitation to Supervise Research).

His main research interests lie in Remote Sensing, 2D signal processing, statistical and spectral analysis applied to ocean surface features detection and characterization. For the last two decades, he has worked in the development of signal and image processing tools for the interpretation of radar signals and the extraction of sea surface features, either natural (wind, waves, currents) or manmade (ships, pollution). These application fields were supported by several European projects and industrial contracts. He is presently engaged in several
initiatives on the topic of Marine Debris and Plastic in the oceans.

Prof. Garello has authored or co-authored more than 60 papers, a hundred and thirty conference communications and three books. He had supervised more than 30 PhD students. For all his works, Prof. Garello was elevated to the grade of Fellow of the IEEE, class of 2006, ``for contributions to signal processing applied to remote sensing of the ocean''.

At IMT Atlantique, Prof. Garello was the head of the research team TOMS (Traitement, Observation et M\'ethodes Statistiques – Processing, Observations and Statistical Methods) within the CNRS unit Lab-STICC before creating the ICTO (ICT for Ocean) program. He is the director of the Scientific Interest Group Bretagne T\'el\'ed\'etection (Brittany Remote Sensing) and leader of the project VIGISAT, a satellite radar receiving ground station for which he obtained twice a multi-million € grant (2009-2014; 2015-2020).

Prof. Garello was an elected IEEE Oceanic Engineering Society AdCom member from 1999 to 2001, from 2003 to 2005 and in 2005 for a new three-year term. In 2005, he was elected Vice-President Conference Operations and then re-elected in 2006 and 2008. In the beginning of 2001, he headed the Committee for defining a new set of Conference Policies and Procedures in order to insure continuity between successive OCEANS conferences. This committee (called JOAB – Joint OCEANS Administrative Board) defined several new approaches and came up with the concept of two Oceans-a-year (every year in Northern America, every other odd year in Europe and every other even year in Asia-Pacific). Prof. Garello was the General Chairman of the first OCEANS of the new Two-Oceans-a-year concept: OCEANS’05 held in Brest, France in June 2005. He received the OES Service Awards in 2006 for developing and implementing the two OCEANS conference policy. In 2012, Prof. René Garello was elected President of the IEEE OES for a two-year term and re-elected
by acclamation in 2014. He is also since 2017 the actual chair of the IEEE Environmental Engineering Initiative, and has been for the last three years seating as principal for IEEE at the GEO (Group on Earth Observation) Executive Committee.

\end{IEEEbiography}

\begin{IEEEbiography}
    [{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/biography/Fablet.jpg}}]{Ronan Fablet} 
graduated with MSc. and Engineer degrees in Space Aeronautics and Applied Math from ISAE/SUPAERO in 1997 and with a PhD in Signal Processing and Computer Vision from University of Rennes/INRIA in 2001. After an INRIA postdoctoral fellowship with Brown University (RI, USA), he was a full-time research scientist at Ifremer (the French Institute for Sea Research) from 2003 to 2007. He joined IMT Atlantique in 2008 and currently holds a Professor position in the Mathematical and Electrical Engineering Department. He has been developing research activities at the interface between signal processing, machine learning and marine science. He has led national and international programs (e.g., EU STREP AFISA, ANR MN EMOCEAN, ANR ASTRID SESAME) and co-authored more than 200 articles and communications in peer-reviewed conferences and journals. His current research interest covers physics-informed deep learning, data-driven approaches to inverse problems, ocean remote sensing and maritime surveillance.

\end{IEEEbiography}
